Algorithms and data structures for first-order logic with connectivity under vertex failures

We introduce a new data structure for answering connectivity queries in undirected graphs subject to batched vertex failures. Precisely, given any graph G and integer k, we can in fixed-parameter time construct a data structure that can later be used to answer queries of the form: ``are vertices s and t connected via a path that avoids vertices $u_1,..., u_k$?'' in time $2^{2^{O(k)}}$. In the terminology of the literature on data structures, this gives the first deterministic data structure for connectivity under vertex failures where for every fixed number of failures, all operations can be performed in constant time. With the aim to understand the power and the limitations of our new techniques, we prove an algorithmic meta theorem for the recently introduced separator logic, which extends first-order logic with atoms for connectivity under vertex failures. We prove that the model-checking problem for separator logic is fixed-parameter tractable on every class of graphs that exclude a fixed topological minor. We also show a weak converse. This implies that from the point of view of parameterized complexity, under standard complexity assumptions, the frontier of tractability of separator logic is almost exactly delimited by classes excluding a fixed topological minor. The backbone of our proof relies on a decomposition theorem of Cygan et al. [SICOMP '19], which provides a tree decomposition of a given graph into bags that are unbreakable. Crucially, unbreakability allows to reduce separator logic to plain first-order logic within each bag individually. We design our model-checking algorithm using dynamic programming over the tree decomposition, where the transition at each bag amounts to running a suitable model-checking subprocedure for plain first-order logic. This approach is robust enough to provide also efficient enumeration of queries expressed in separator logic.

==> aggregators.tex <==
\section{Nested aggregators\sz{this is unused}}
An \emph{aggregator} is a function $a\from \prod_{i\in I}X_i\to X$,
where 
 $(X_i)_{i\in I}$ is a family of sets and $X$ is a set and $\prod_{i\in I}X_i$ is its Cartesian product.
 The \emph{aggregator query problem} for an aggregator $a$ is the following query problem.\\


\noindent 
\textbf{Input:} a tuple $\tup x=(x_i)_{i\in I}\in \prod_{i\in I} X_i$\\
\textbf{Query input:} a tuple $\tup y=(y_i)_{i\in J}\in \prod_{i\in J} X_i$, where $J\subset I$\\
\textbf{Output:} $a(\tup x\ast \tup y)$ 
where $\tup x\ast \tup y$ is the tuple obtained from $\tup x$ by overwriting the entries at the positions in $J$ according to $\tup y$.\\


If $(a_v)_{v\in V}$ is a family of aggregators
where $a_v\from \prod_{i\in I_v}X_i^v\to X_v$
and $a\from \prod_{v\in V} X_v\to X$ is another aggregator,
then we can compose the aggregators, yielding an aggregator
$a'\from 
\prod_{v\in V,i\in I_v}X_i^v\to X$. 
By iteratively composing aggregators we compose an entire tree of aggregators, as follows.

A \emph{tree of aggregators} is a 
 tree $T$ in which each node $v$ is labelled with a set $X_v$ 
and with each inner node $v$ an aggregator \[a_v\from \left(\prod_{\text{$w$ child of $v$}}X_w \right)\to X_v\]
is associated.
Composing the aggregators iteratively yields the \emph{nested aggregator}
\[a_T\from \left(\prod_{\text{$w$ leaf of $T$}}X_w \right)\to X_r,\]
where $r$ is the root of $T$.
It's value on a tuple $\tup x$ 
is defined inductively. Namely, 
for each node $v$ of $T$
define the value $v(\tup x)\in X_v$ 
as follows:
\begin{itemize}
  \item if $v$ is a leaf then $v(\tup x)=\tup x(v)$,
  \item otherwise, if $v$ is an inner node with children $W$ and aggregator $a_v$ then the value $w(\tup x)$ has already been defined for every child $w\in W$ of $v$,
   and  $v(\tup x)$ is defined as $a_v((w(\tup x))_{w\in W})$.
\end{itemize}
Then $a_T(\tup x)$ is defined as $r(\tup x)$ where $r$ is the root of $T$.

The following theorem implies that if a tree $T$ is composed of aggregators with constant query time, then the aggregator $a_T$ also has constant query time. It therefore allows to speed up the naive query evaluation of a tree of aggregators to constant time.

\begin{theorem}\label{thm:tree aggregator}
  Let $T$ be a tree of aggregators with $|X_v|\le r$ for all nodes $v$ of $T$,
  and suppose the aggregator $a_v$ at node $v$ has a query answering algorithm with initialization time $t_v$ and query answering time $t_v'(k)$ for queries of length $k$.
  Then the nested aggregator $a_T$ has a query answering algorithm with initialization time \[O_r\left(\sum_{v\in V(T)}\left(t_v+ t_v'(1)\right)\right)\]
  and query answering time \[k\cdot O_r\left(\max_{v\in V(T)}t_v'(k)\right)\]{}
  for queries of length $k$.
  In particular, if $t_v$ is linear in the number of children of $v$ and $t'_v(k)=O_k(1)$ then 
  the query answering algorithm for $a_T$ has initialization time linear in $|V(T)|$ and query answering time $O_{k,r}(1)$.
\end{theorem}
\begin{proof}
  In the initialization phase, 
  input a tuple $\tup x$ 
  and 
  compute the output value $x_v:=v(\tup x)$ by proceeding from the leaves towards the root as in the definition of $v(\tup x)$.
  More precisely, 
  at a leaf $v$, the value $x_v\in X_v$ is the appropriate component of the input tuple $\tup x$ given in the initialization.
  To compute $x_v$ for an inner node $v\in V(T)$, initialize the aggregator $a_v$ on input $\tup x_v:=(x_w)_{w\in W}$ where $W$ is the set of children of $v$, and query it with the empty query, yielding the value $x_v:=a_v((x_w)_{w\in W})=v(\tup x)$.

  For each node $w$ with parent $v$
  define the function $f_{wv}\from X_w\to X_v$ such that 
  $f_w(x)=a_v(\tup y)$ 
  where $\tup y\in \prod_{\text{$u$ child of $v$}}X_u$ 
  is such that $\tup y(u)=x_u$ for every child of $v$ other than $w$,
  and $\tup y(w)=x$.
The function $f_{wv}$ can be computed in time $r\cdot t'_v(1)$, by performing $r$ queries to the aggregator $a_v$.

% For each $v$ let $\hat X_v:=2^{X_v}$ and 
% for an edge $vw$
% define $F_{vw}\from \hat X_v\to\hat X_w$ by $f_{w}^{-1}\from 2^{X_v}\to 2^{X_w}$.
Initialize a reverse tree-function composer for the tree $T$ in which each vertex is labeled by $X_v$ and each edge $vw$ is labeled with the function $f_{wv}\from X_w\to X_v$.
Furthermore, initialize the data structures answering the least common ancestor and direction queries, as given by~\cref{lem:navigation}.

This completes the initialization phase, whose duration is as in the statement.

\medskip
We now describe the query answering phase.
Let $\tup y=(y_w)_{w\in R}$ be given, where $R$ is a set of leaves and 
$y_w\in X_w$ for each $w\in R$.
Compute the least common ancestor  closure $R'\supseteq R$ of $R$ and additionally add the root of $T$ to $R'$.
For each $w\in R'$ other than the root
let $v$ be the 
 immediate predecessor of $w$ in $(R',\preceq)$.
 Call the node $\dir(v,w)$ the \emph{proxy} of $w$.
 Hence, for every $v\in R'$, the set of immediate successors $w$ of $v$ in $(R',\preceq)$ is mapped injectively by the proxy function to 
 the children of $v$ (see Fig.~\ref{fig:lca-closure}).
 \begin{figure}[h]
  \centering
  \includegraphics[scale=0.5]{lca.pdf}
  \caption{The sets $R,R'$ and $R''$.\textcolor{red}{Sz: fix font}}  
  \label{fig:lca-closure}
 \end{figure}
Let $R''$ be the set of proxies of all nodes in $R'$.
The sets $R'$ and $R''$ as well as the proxy function can be computed in time $O(|R|)$ using the data structure from~\cref{lem:navigation}.

\medskip
Fix a node  $u\in R'$ other than the root and its proxy $u'\in R''$.
Let $f_{uu'}\from X_{u}\to X_{u'}$ be the composition of the functions $f_{wv}$ labelling the edges $vw$ along the path from $u$ to $u'$
(if $u=u'$ then $f_{uu'}$ is the identity on $X_u$).
Then the function $f_{uu'}$ can be obtained by a query to the reverse tree-function composer. 
% We show how to compute the function $f_{uu'}$ using our data structure.

% Let $F_{u'u}$ be the composition of the functions $F_{vw}$ along  the path from $u'$ to $u$.
% Then $F_{u'u}\from 2^{X_{u'}}\to 2^{X_{u}}$ can be computed using the tree-function composer.
% Moreover, $F_{u'u}=f_{uu'}^{-1}$, so $f_{uu'}$ can be computed from $F_{u'u}$.



For every node $v$ of $T$ define the ``updated value'' $y_v$ as $y_v:=v(\tup x\ast \tup y)$. Our goal is to compute the value $y_r$ where $r$ is the root.

We show how to compute $y_v$ for every node $v\in R'\cup R''$, by proceeding from the leaves towards the root.
If $v\in R$ then $v$ is a leaf in $T$ and $y_v$ is the appropriate component of the tuple $\tup y$ given as the input to the query.
If $u'\in R''$ is a proxy of $u\in R'$ 
and $y_u$ is already defined then $y_{u'}:=f_{uu'}(y_u)$,
and this value can be computed by querying the reverse tree-function composer.

Suppose now that $v\in R'$ is an inner node with children $W$.
Let $\tup x_v=(x_w)_{w\in W}$ be the tuple with which the aggregator $a_v$ was initialized.
Consider the tuple $\tup y_v$ indexed by $W\cap R''\subset W$,
such that the $w$-component of $\tup y_v$ is equal to $y_w$, which was computed earlier since $w\in R''$. Then $y_v=a_v(\tup x_v\ast \tup y_v)$.
The value $y_v$ can be therefore computed by querying the aggregator $a_v$ with the tuple $\tup y_v$.

This way, we compute $y_v$ for every $v\in R'\cup R''$,
using $O(|R|)$ queries to the data structures computed during initialization.
The value $y_r$ at the root $r$ of $T$ is then the answer to the query.
\end{proof}
\medskip

\textcolor{red}{Sz: it remains to show that for each node $v$ of the bag graph there is an aggregator 
$a_v$ which given 
the profile of every child of $v$ outputs the profile of $v$.
The initialization time of $a_v$ is linear in the number of children and the query time is constant. \cref{thm:general-queries} then follows from \cref{thm:tree aggregator}.
}

Let $G$ be the input graph. 
Construct the (regular) tree decomposition $\Tt$ using the algorithm of
  \cref{thm:strong-unbreakability}, with underlying tree $T$.
  
  Suppose we want to answer a query $\conn(s,t,S)$, where $s,t\in V(G)$ and $S$ is a vertex subset of size at
most $k$.  
%Let $\Sh\coloneqq S\cup \{u,v\}$. Note that $|\Sh|\leq k+2$.

Let $s_*$ and $t_*$ be two symbols
formally representing $s$ and $t$.
For $v\in V(T)$, let
$D(v)$ be the adhesion of $v$ 
extended by $s_\ast$ if $s\in\cone(x)$ and by $t_\ast$ if $t\in\cone(x)$.

The {\em{profile}} of $x$ is the set
$\profile(x)\subseteq\binom{D(x)}{2}$ consisting of all pairs
$\set{a,b}\in \binom{D(x)}{2}$ satisfying the following condition: in
$G[\cone(x)]$ there is an $a$-$b$ path that does not pass through any
vertex of $S$, where $s_*$ and $t_*$ are interpreted as $s$ and $t$, respectively.

Let $r$ be the root of $T$. Then $D(r)=\set{s_*,t_*}$ and $\profile(r)$ is
non-empty if and only if \mbox{$G\models \conn(s,t,S)$}. Therefore, it
suffices to compute the profile of the root, $\profile(r)$. 


For each node $v$ let 
 $X_v$ be the set of all subsets of $\binom{D(x)}{2}$.
 Then $\profile(v)\in X_v$.

 \begin{lemma}Fix an inner node $v$ of $T$ with children $W$. There is
  an aggregator 
  $a_v\from \prod_{w\in W}X_w\to X_v$ 
  independent of $s,t$ and $S$ such that for any fixed $s,t$ and $S$ with $|S|\le k$, 
  $a_v(\tup x)=\profile(v)$ 
  if $\tup x$ is the tuple such that $\tup x(w)=\profile(w)$ for each $w\in W$.
  Moreover, there is a query answering algorithm for $a_v$ with initialization time ... and update time ...
 \end{lemma}
  \begin{proof}
    \textcolor{red}{The proof is essentially in \cref{lem:aggregate}}, but needs to be adapted.
  \end{proof}







==> app-enumeration.tex <==
% !TEX root = main.tex

\section{Proof of \cref{lem:automata enumeration}}\label{sec:automata enumeration}

We now prove \cref{lem:automata enumeration}, which we repeat for
convenience. 

\lemenum*

Fix an automaton $\aut A$ over the alphabet $A\otimes \tup x$, and let $Q$ be its set of states.
A \emph{shape} $\sigma$ consists of the following:
\begin{itemize}
  \item a set of variables $\tup y$ contained in $\tup x$,
  \item a rooted tree $S$, with the root denoted $\ast$;
  % \item a labelling assigning states from $Q$ to edges of $S$,
  \item a labeling $L\colon V(S)\cup E(S) \to Q$ assigning states from $Q$ to vertices and edges of $S$,
  \item a valuation $\tup s\from \tup y\to V(S)$
  such that every node in $S$ is either in the image of $\tup s$, or is the least common ancestor of some two nodes in the image of $\tup s$.
\end{itemize}

% A \emph{non-branching shape} $\sigma$ is defined similarly, except that
% the root $\ast$ has one child, and the edge joining it with $\ast$ has no label in $Q$.
% A \emph{shape} is either a branching shape or a non-branching shape.

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.45\linewidth}
    \centering
    \begin{tikzpicture}
      \node (v0) at (2,3) [circle,draw,label=left:\textcolor{blue}{$q_1$},label=right:$\ast$,scale=0.7] {};
      \node (v1) at (0,1.5) [circle,draw,label=left:\textcolor{blue}{$q_2$},scale=0.7] {};
      \node (v2) at (3.75,1.5) [circle,draw,label=left:\textcolor{blue}{$q_4$},label=right:$\tup s(x_4)$,scale=0.7] {};
      \node (v3) at (-1.5,0) [circle,draw,label=left:\textcolor{blue}{$q_1$},label=below:$\tup s(x_2)$,scale=0.7] {};
      \node (v4) at (0,0) [circle,draw,label=left:\textcolor{blue}{$q_1$},scale=0.7] {};
      \node (v5) at (1.5,0) [circle,draw,label=left:\textcolor{blue}{$q_4$},label=below:$\tup s(x_7)$,scale=0.7] {};
      \node (v6) at (3,0) [circle,draw,label=left:\textcolor{blue}{$q_3$},label=below:$\tup s(x_5)$,scale=0.7] {};
      \node (v7) at (4.5,0) [circle,draw,label=left:\textcolor{blue}{$q_6$},label=below:$\tup s(x_6)$,scale=0.7] {};
      \node (v8) at (-.75,-1.5) [circle,draw,label=left:\textcolor{blue}{$q_2$},label=below:$\tup s(x_1)$,scale=0.7] {};
      \node (v9) at (.75,-1.5) [circle,draw,label=left:\textcolor{blue}{$q_3$},label=below:$\tup s(x_3)$,scale=0.7] {};

      \draw (v0) -- (v1) node[midway,yshift=4,xshift=-4,blue] {$q_7$};
      \draw (v0) -- (v2) node[midway,yshift=4,xshift=4,blue] {$q_5$};
      \draw (v1) -- (v3) node[midway,yshift=4,xshift=-4,blue] {$q_5$};
      \draw (v1) -- (v4) node[midway,yshift=0,xshift=-5,blue] {$q_1$};
      \draw (v1) -- (v5) node[midway,yshift=4,xshift=4,blue] {$q_6$};
      \draw (v2) -- (v6) node[midway,yshift=1,xshift=-6,blue] {$q_2$};
      \draw (v2) -- (v7) node[midway,yshift=1,xshift=6,blue] {$q_7$};
      \draw (v4) -- (v8) node[midway,yshift=1,xshift=-6,blue] {$q_4$};
      \draw (v4) -- (v9) node[midway,yshift=1,xshift=6,blue] {$q_5$};
    \end{tikzpicture}
    \subsection*{$S$}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\linewidth}
    \centering
    \begin{tikzpicture}
      \node (v0) at (2,3) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_1$}},label=right:$\ast$,scale=0.7] {};
      \node (v10) at (1,2) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_7$}},scale=0.7] {};
      \node (v11) at (2.875,2) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_5$}},scale=0.7] {};
      \node (v1) at (0,1) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_2$}},scale=0.7] {};
      \node (v12) at (-.75,0) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_5$}},scale=0.7] {};
      \node (v13) at (0,0) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_1$}},scale=0.7] {};
      \node (v14) at (.75,0) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_6$}},scale=0.7] {};
      \node (v2) at (3.75,1) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_4$}},label=right:$\tup a(x_4)$,scale=0.7] {};
      \node (v15) at (3.375,0) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_2$}},scale=0.7] {};
      \node (v16) at (4.125,0) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_7$}},scale=0.7] {};
      \node (v3) at (-1.5,-1) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_1$}},label=below:$\tup a(x_2)$,scale=0.7] {};
      \node (v4) at (0,-1) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_1$}},scale=0.7] {};
      \node (v17) at (-.375,-2) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_4$}},scale=0.7] {};
      \node (v18) at (.375,-2) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_5$}},scale=0.7] {};
      \node (v5) at (1.5,-1) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_4$}},label=below:$\tup a(x_7)$,scale=0.7] {};
      \node (v6) at (3,-1) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_3$}},label=below:$\tup a(x_5)$,scale=0.7] {};
      \node (v7) at (4.5,-1) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_6$}},label=below:$\tup a(x_6)$,scale=0.7] {};
      \node (v8) at (-.75,-3) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_2$}},label=below:$\tup a(x_1)$,scale=0.7] {};
      \node (v9) at (.75,-3) [circle,draw,label={[xshift=-9,yshift=-10]\textcolor{blue}{$q_3$}},label=below:$\tup a(x_3)$,scale=0.7] {};

      \path (v0) edge (v10)
            (v0) edge (v11)
            (v10) edge (v1)
            (v11) edge (v2)
            (v1) edge (v12)
            (v1) edge (v13)
            (v1) edge (v14)
            (v2) edge (v15)
            (v2) edge (v16)
            (v12) edge (v3)
            (v13) edge (v4)
            (v14) edge (v5)
            (v15) edge (v6)
            (v16) edge (v7)
            (v4) edge (v17)
            (v4) edge (v18)
            (v17) edge (v8)
            (v18) edge (v9);
    \end{tikzpicture}
    \subsection*{$T$}
  \end{subfigure}
  \caption{Examples of a shape and embedding of shape}
  \label{fig:shape}
\end{figure}

% For a node $v\in S$ and $x,y\in \tup y$ we write $v=\textrm{lca}(x,y)$
% if $v$ is the least common ancestor of $\tup s(x)$ and $\tup s(y)$.
%Thanks to the last condition above, every node $v\in S$ (save perhaps the root) is of the form $\textrm{lca}(x,y)$ for some $x,y\in \tup y$. In particular, $S$ has at most $2|\tup y|$ nodes, and we obtain the following.

Thanks to the last condition above $S$ has at most $2|\tup y|-1$ nodes, and we obtain the following.

\begin{lemma}\label{lem:shapes}Fix $\tup y\subset \tup x$.
    The set of shapes with variables $\tup y$ is finite, and can be effectively computed, given~$\aut A$.
\end{lemma}


Fix a tree $T$ over the alphabet $A$, a shape $\sigma$ as above, a valuation $\tup a\from \tup y\to V(T)$,
and let $\rho\from V(T)\to Q$ be the (unique) run of $\aut A$ on $T\otimes \tup a$.
The valuation $\tup a$ \emph{matches} $\sigma$ with \emph{starting node} $v\in V(T)$ if there is a function $F\from V(S)\to V(T)$ such that:
\begin{enumerate}
  \item $F$ preserves least common ancestors, that is, for all $a,b,c\in V(S)$, if $c$
  is the least common ancestor of $a$ and $b$ in $S$ then $F(c)$ is the least common ancestor of $F(a)$ and $F(b)$ in $T$. In particular, $F$ preserves $\preceq$.
  \item $F$ is injective,
  \item  $F(\tup s)=\tup a$, that is, $F(\tup s(x))=\tup a(x)$ for every $x\in \tup y$,
  \item $F(\ast)=v$, where $\ast$ is the root of $S$,

  \item for every vertex $w$ of $S$, $\rho(F(w))= L(w)$,
  \item for every edge $e=ww'$ of $S$ between a node $w$ and its child $w'$, the
  $F(w')$-directed child of $F(w)$ in $T$ satisfies $\rho(v')=L(e)$.
%  \textit{\small(Recall from the preliminaries that the $F(w')$-directed child of $F(w)$ is the only child of $F(w)$ that is an ancestor of $F(w')$ in $T$).}

%   there is $v'\in V(T)$ that is, a child of $F(v)$, an ancestor of $F(w)$, and such that $\rho(v')=L(e)$.
\end{enumerate}

Note that if $\bar a$ matches $\sigma$, then the function
$F$ witnessing this is unique. Moreover, no valuation~$\tup a$ matches two distinct shapes,
since the rooted tree $S$ and the labeling $L$ of its nodes and edges is uniquely determined by the valuation $\tup a$ and the unique run of $\aut A$ on $T\otimes \tup a$.

\medskip
Fix a shape $\sigma$. Our next goal is to
compute for each possible starting node $v$ an enumerator
for the set of all valuations $\tup a$ that match the shape $\sigma$ with starting node~$v$.

%Our goal is to compute an enumerator for the set of all starting nodes $v\in V(T)$ for~$\sigma$,
%and for each such node $v$, enumerate the set of all valuations   $\tup a$ that match the shape and have~$v$ as their starting node.

\begin{lemma}\label{lem:shape enumeration}
    For every shape $\sigma$ there is a constant $c$ computable from $\aut A$ and $\sigma$, and an algorithm that, given a tree~$T$ over the alphabet $A$, computes
    in time  $c\cdot |T|$ a collection $(\mathcal E_v)_{v\in V(T)}$ of enumerators,
    where for each $v\in V(T)$,  $\mathcal E_v$ is
    an enumerator with delay $c$ for the set of all valuations $\tup a$ that match $\sigma$ with starting node $v$.
\end{lemma}

We first show how~\cref{lem:shape enumeration} implies~\cref{lem:automata enumeration}.
\begin{proof}
Let $\CC$ be a class of structures for which enumeration of
$\FO(\Sigma\cup A)$ queries is efficient for every finite alphabet $A$.
Let $\aut A$ be an automaton on augmented trees over an  alphabet
of the form $A\otimes \tup x$ and let $T$ be a $\CC$-augmented tree over the alphabet $A$.
We extend $\tup x$ to $\tup x\cup\set{z}$ by adding a dummy variable~$z$.
We view
$\aut A$ as an automaton over the alphabet $A\otimes (\tup x\cup \{z\})$. Using~\cref{lem:shapes}, compute the set~$\Delta$ of all shapes $\sigma$ in which the root node of the shape carries the variable
$z$ (that is, $\tup s(z)=\ast$) and
is labeled with an accepting state of $\aut A$ (that is, $L(\ast)$ is an accepting state). For each such shape $\sigma$ compute
the enumerator $\aut E_r^\sigma$ for the set of all valuations $\tup a\from \tup z\cup \set{r}\to V(T)$ that
match $\sigma$ with starting node $r$, where $r$ is the root of $T$. This is possible in time linear
in $|T|$ by~\cref{lem:shape enumeration}.

An enumerator for $\aut A(T)$ as in the statement of~\cref{lem:automata enumeration}
is obtained
by concatenating the enumerators $\aut E_r^\sigma$ for all the shapes $\sigma\in \Delta$,
where each output $\tup a\from \tup x\cup \set{r}\to V(T)$ of each of those enumerators is post-processed by projecting it
to a valuation $\tup a'\from \tup x\to V(T)$, that is, by removing
the entry corresponding to the dummy variable.

 As remarked above (see comment following the definition of matching a shape), for distinct shapes the sets of valuations that
match the shapes are disjoint.
Hence, all valuations are enumerated without
repetition.  By choosing $f$ appropriately this
yields an enumerator that is computable in time $f(|\phi|)\cdot |T|$
and has delay~$f(|\phi|)$.
\end{proof}

We will need the following lemmas regarding enumeration of specific sets on unranked trees.

\medskip
For a set $U$ of nodes of a tree $T$ and two nodes $v,w$, say that $w$ is a \emph{minimal} descendant of $v$ in $U$ if $w\in U$, $w$ is a descendant of $v$, 
and no inner node of the path from $v$ to $w$ belongs to $U$.

\begin{lemma}\label{lem:minimal-descendants}
  There is a constant $c$ and an algorithm that, given a tree $T$ and a set $U$ of its nodes, computes in time $c\cdot |T|$ a collection $(\mathcal E_v)_{v\in V(T)}$ 
  of enumerators, where for each $v\in V(T)$,  $\mathcal E_v$ is
    an enumerator with delay $c$ for the set of minimal descendants $w$ of $v$ that belong to $U$.
\end{lemma}
\begin{proof}\newcommand{\pr}{<_{\text{pre}}}
Assume without loss of generality that the root of $T$ belongs to $U$.
Let $\pr$ denote the order on~$V(T)$ obtained by performing a pre-order traversal of $T$.

For each node $v$ of $T$ let $M_v$ denote the set of all the minimal descendants of $v$ that belong to $U$,
and let $g(v)$ denote the $\preceq$-largest ancestor of $v$ that belongs to $U$ (with $g(v)=v$ if $v\in U$).
Note that $M_v=M_{g(v)}$ for every node $v$ of $T$.

Note that we can compute the function $g$ in time $\Oh(|T|)$
(represented say as pointers from $v$ to~$g(v)$) by performing a depth-first search traversal of $T$.
Moreover, again by performing a depth-first search traversal, we can compute, for each $v\in U$ and jointly in time $\Oh(|T|)$,
a linked list enumerating all elements of $M_v$.

Now, to obtain an enumerator for $M_v$ given a node $v$ of $T$, first compute $g(v)$ and then follow the list enumerating the elements of $M_{g(v)}$. Since $M_v=M_{g(v)}$, this enumerates $M_v$, with constant delay. 
\end{proof}

\begin{lemma}\label{lem:enumerate}
  Fix a finite set $Q$ of size $q$
  and two elements $x,y\in Q$.
  There is a constant $c$ depending only on $q$ and an algorithm that, 
  given a tree $T$ in which each edge $vw$ is labeled by a function $f_{vw}\colon Q\to Q$, computes in time $c\cdot |T|$ a collection 
  $(\mathcal E_v)_{v\in V(T)}$ 
  of enumerators, where for each $v\in V(T)$,  $\mathcal E_v$ is
    an enumerator with delay $c$ that enumerates all descendants $w$ of $v$ such that the composition of the functions labeling the edges of the path from $v$ to $w$ maps $x$ to $y$.
\end{lemma}
\begin{proof}
For two nodes $v,w$ with $v\preceq w$ let $f_{vw}$ denote the composition of the functions labeling the edges of the path from $v$ to $w$.
Let $D_v^{xy}$ be the set of all strict descendants $w$ of $v$ such that $f_{vw}(x)=y$, and 
let $M_v^{xy}\subset D_v^{xy}$ be the set of \emph{minimal}
such descendants, where $w$ is minimal if there is no $u\in D_v^{xy}$ with $v\prec u\prec w$.

  It suffices to compute, for each $v\in V(T)$, an enumerator
  for the set $M_v^{xy}$. Indeed, the enumerator for $D_v^{xy}$ can be then obtained by enumerating all nodes $w\in M_v^{xy}$
  and then, for each such $w$,
  recursively enumerating the set 
  $D_w^{yy}$.

Proceeding from the root of $T$ towards the leaves, for
   each node $v$ of $T$ construct an injective coloring function
   $c_v\from Q\to [q]$, so that the following property holds:
   \[c_v(f_{vw}(x))\le c_w(x)\qquad\text{for every edge $vw$ and all
     $x\in Q$}.\] This can be done as follows.  At the root $v$,
   pick an arbitrary injection $c_v\from Q\to [q]$. If $c_v$ is
   defined for some node $v$ and $w$ is its child, then first define
   $c_{w}\from f_{vw}(Q)\to [q]$ by setting $c_w(y)$, for
   $y\in f_{vw}(Q)$, to the least color $c\in [q]$ such that
   $c_v(x)=c$ for some $x\in Q$ with $f_{vw}(x)=y$. Next, extend
   $c_w$ to an injection $c_w\from Q\to [q]$ arbitrarily.  The
   required property then holds by construction.  The computation of
   the colorings $c_v$ therefore takes time $\Oh(|T|\cdot r)$.

%  Apply the coloring procedure from the proof of \cref{thm:function composer}, obtaining in linear time for each node $v$ of $T$   an injective coloring function $c_v\from X\to [r]$ such that 
%  \[c_v(f_{vw}(x))\le c_w(x)\qquad\text{for every edge $vw$ and all $x\in X$}.\]


  For every $y\in Q$ and color $c\in [q]$ let $C[y/c]$ denote the 
set of nodes $v$ such that $c_v(y)=c$.

  We describe how to compute in time $\Oh_r(|V(T)|)$ a collection of constant-delay enumerators $\mathcal E_v^{xyd}$ for the set $M_v^{xy}\cap C[y/d]$, for all $x,y\in Q$, $d\in [q]$ and all nodes $v\in V(T)$.
  Then an enumerator for~$M_v^{xy}$ can be obtained by concatenating the enumerators $\mathcal E_v^{xyd}$ for all $d\in [q]$.

  Fix elements $x,y\in Q$ and colors $c,d\in [q]$. Our goal now is to compute (in time $\Oh_r(|V(T)|)$) constant-delay enumerators 
  for each of the sets $M_v^{xy}\cap C[y/d]$, for all nodes $v\in C[x/c]$. Since the sets $(C[x/c])_{c\in [q]}$ partition $V(T)$, this will jointly give all the required enumerators.
  Assume in what follows that $v\in C[x/c]$.
  


Let $F_c\subset E(T)$ be the set of those edges $vw$ in $T$ such that 
$f_{vw}$ maps the element of color $c$ to an element of smaller color.
The set $F_c$ can be computed in time  $\Oh_r(|V(T)|)$.
Write $v\sim_c w$ if the path between two nodes $v$ and $w$ does not contain any edge from $F_c$.
Furthermore, compute in time $\Oh_r(|V(T)|)$ the set $C[y/d]$.

Fix a node $v\in C[x/c]$.
If $c<d$, then $M_v^{xy}\cap C[y/d]=\emptyset$.
If $c=d$, then for every descendant $w$ of $v$
we have $w\in M_v^{xy}\cap C[y/d]$ if and only if 
  $v\sim_cw$, $w\in C[y/d]$ and 
  no inner node of the path from $v$ to $w$ belongs to $C[y/d]$.
Consider the rooted forest $T-F_c$ obtained from $T$ by removing the edges in $F_c$, where the root of each tree in the forest is the its smallest node with respect to the ancestor relation in $T$.
By considering each tree in this forest separately,
the problem is solved by the algorithm from~\cref{lem:minimal-descendants} applied to that tree and the set $C[y/d]$ restricted to that tree.



We are left with the case when $c>d$.
We proceed by induction on $c-d$.

\medskip
Compute the set $U$ of all nodes $u$ of $T$ with the following properties:
\begin{itemize}
  \item $u$ is the lower endpoint of an edge $u'u$ in $F_c$,
  \item $M_w^{x'y}\cap C[y/d]$ is non-empty,
  where 
  $x'=f_{u'u}(z)$ and $z\in Z$ is such that $c_{u'}(z)=c$. 
\end{itemize}
Note that as the edge $u'u$ is in $F_c$ it follows that $c_u(x')<c$,
and we can apply the inductive assumption, thus assuming that 
each node $u$ is equipped with a constant-delay enumerator for $M_u^{x'y}\cap C[y/d]$, for all $x'\in Q$. In particular we can test whether $M_u^{x'y}\cap C[y/d]$ is non-empty in constant time, and so the set $W$ can be computed in linear time. 

The following conditions are equivalent for a node $v\in C[x/c]$
and its descendant $w$:
\begin{itemize}
  \item $w\in M_v^{xy}\cap C[y/d]$,
  \item $v$ has some minimal descendant $u\in U$ such that $w\in M_u^{x'y}\cap C[y/d]$, where $x'$ is as above.
\end{itemize}
It follows that $M_v^{xy}\cap C[y/d]$
is the disjoint union, over all minimal descendants $u\in U$ of $v$,
of the (non-empty) set 
$M_u^{x'y}\cap C[y/d]$, where $x'$ is as above.
Hence, an enumerator for $M_v^{xy}\cap C[y/d]$
can be obtained by first enumerating all minimal descendants $u\in U$ of $v$ using the data structure from~\cref{lem:minimal-descendants}, and then, for each such $u$,
using the enumerator for $M_u^{x'y}\cap C[y/d]$ obtained by inductive assumption. 
\end{proof}

In our application, we will  need to compose the functions in the reverse order. Hence the following.



\begin{lemma}\label{lem:reverse enumerate}
  Fix a finite set $Q$ of size $q$
  and two elements $x,y\in Q$.
  There is a constant $c$ depending only on $q$ and an algorithm that, 
  given a tree $T$ in which each edge $vw$ is labeled by a function $f_{vw}\colon Q\to Q$, computes in time $c\cdot |T|$ a collection 
  $(\mathcal E_v)_{v\in V(T)}$ 
  of enumerators, where for each $v\in V(T)$,  $\mathcal E_v$ is
    an enumerator with delay $c$ that enumerates all descendants $w$ of $v$ such that the composition of the functions labeling the edges of the path from $w$ to $v$ maps $x$ to $y$.
\end{lemma}
\begin{proof}
%  As in~\cref{cor:reverse tree-function composer}.
     A function $f\from X\to Y$ is uniquely determined by its inverse
     $f^{-1}\from 2^Y\to 2^X$. Moreover, this preserves compositions:
     $(f\circ g)^{-1}=g^{-1}\circ f^{-1}$.  We can therefore apply \cref{lem:enumerate}
     to $T$ where each edge $vw$ is labeled with
     $f_{vw}^{-1}$.
\end{proof}

In the remainder of this section we prove~\cref{lem:shape enumeration}.
Fix an augmented tree $T$ and let $\rho_0$ be the run of $\aut A$ on $T\otimes \emptyset$.
For a node $w\in V(T)$ and state $p\in Q$, let $\rho_0[w\mapsto p]$
be the labeling that assigns states from $Q$ to nodes of $T$ such that
\begin{itemize}
\item $\rho_0[w\mapsto p]$ agrees with $\rho_0$ on nodes that are not ancestors of $w$,
\item $\rho_0[w\mapsto p]$ maps $w$ to $p$, and
\item $\rho_0[w\mapsto p]$ inductively maps a strict ancestor
$w'$ of $w$
to a state $q$ such that
$\delta_{q,(a,\emptyset)}$ holds in the whorl of $w'$ labeled by $\rho_0[w\mapsto p]$.
\end{itemize}

 In other words, $\rho_0[w\mapsto p]$ is obtained from $\rho_0$ by enforcing the state at $w$ to be $p$,
and otherwise continuing with the bottom-up evaluation of $\aut A$ on $T\otimes \emptyset$. If $w'$ is a node of $T$, then write \mbox{$[w\mapsto p]\vdash [w'\mapsto p']$} if $\rho_0[w\mapsto p]$ labels $w'$ with $p'$.
    

\begin{lemma}\label{lem:state entailment}
    Fix states $q_1,q_2\in Q$.
%    There is an algorithm that,
%    given a tree $T$ and a set $X\subset V(T)$,
%    in time linear in $|T|$ computes, for each vertex $v\in V(T)$ two enumerators with constant delay.
%    The first one enumerates all children $u_1$ of $v$ that have some descendant $u_2\in X$ such that $[u_2\mapsto q_2]\vdash [u_1\mapsto q_1]$.
%    The second one enumerates  all descendants $u_2\in X$ of $v$ such that $[u_2\mapsto q_2]\vdash [v\mapsto q_1]$.
  There is a constant $c$ and an algorithm that, 
  given a tree $T$ and a set $X\subseteq V(T)$ computes in time $c\cdot |T|$ two collections 
  $(\mathcal E_v)_{v\in V(T)}$ and $(\mathcal E'_v)_{v\in V(T)}$ 
  of enumerators with delay~$c$, doing the following: For each $v\in V(T)$,  $\mathcal E_v$ is
    an enumerator that enumerates all children $u_1$ of~$v$ that have some descendant $u_2\in X$ such that $[u_2\mapsto q_2]\vdash [u_1\mapsto q_1]$. 
    For each $v\in V(T)$,  $\mathcal E'_v$ is
    an enumerator that enumerates all descendants $u_2\in X$ of $v$ such that $[u_2\mapsto q_2]\vdash [v\mapsto q_1]$.
\end{lemma}
\begin{proof}
We let $Q'\coloneqq Q\mathop{\dot\cup} \{m,0,1\}$. We label each edge $vw$ of $T$ by the 
function $f_{wv}\from Q'\rightarrow Q'$ such that 
\begin{itemize}
\item 
$f_{wv}(p)=q$ if $[w\mapsto p]\vdash [v\mapsto q]$, for all $p,q\in Q$, 
\item $f_{wv}(m)=1$ if 
$w\in X$ and $f_{wv}(m)=0$ if $w\not\in X$, and
\item   $f_{wv}(0)=0$, and $f_{wv}(1)=1$.
\end{itemize}

Observe that if $w$ is any descendant of $v$, then $[w\mapsto p]\vdash [v\mapsto q]$  if and only if the composition of the functions labeling the edges along the path from $w$ to $v$ is a function $f$ such that $f(p)=q$. Furthermore, this function 
maps $m$ to $1$ if and only if $w\in X$. 

We now apply \cref{lem:reverse enumerate} to apply in the claimed time
the second collection $(\mathcal E'_v)_{v\in V(T)}$ of enumerators with the
desired properties. 

We now compute the set $Y$ of 
all vertices $v$ that have a descendant $u\in X$ such that 
$[u\mapsto q_2]\vdash [v\mapsto q_1]$. For this, we 
iterate over all $v\in V(T)$ and let $\mathcal{E}'_v$ enumerate
its first output. If $\mathcal{E}'_v$ does not report an error, 
there exists a descendant $u\in X$ of $v$ such that 
$[u\mapsto q_2]\vdash [v\mapsto q_1]$. Assuming that each 
enumeration takes a constant time $c'$, we can compute
this set in time $c'\cdot |T|$. Now it is easy to construct 
the first collection $(\mathcal E_v)_{v\in V(T)}$ 
of enumerators with the desired properties (compare with 
the more complicated construction in the proof of 
\cref{lem:minimal-descendants}). 
%
%
%We extend $T$ by unary predicates uniquely marking $v$ and the
%set $X$. We state an MSO formula~$\psi(x)$ over the extended 
%vocabulary with the property that
%$T\models \psi(u_1)$ if and only if $u_1$ is a child of~$v$ that has some descendant $u_2\in X$ such that $[u_2\mapsto q_2]\vdash [u_1\mapsto q_1]$. In~$\psi(x)$ we verify that $y$ is a child of $v$ by quantifying
%the unique element that is marked by the predicate marking $v$. 
%We then existentially quantify 
%the descendant $y$ of $x$ and the states of the unique
%run $\rho_0[y\mapsto q_2]$ and ensure with the formula 
%that the run indeed follows the transitions of the automaton. 
%We then require that $x$ is labeled with $q_1$.
%
%Now the claim concerning the first enumerator follows from the fact that we can enumerate
%MSO properties over trees with constant delay, see 
%\cite[Theorem 2.3]{KazanaS13}. 
%
%Regarding the second enumerator, we reduce it to the  problem considered in \cref{lem:reverse enumerate}.
%Label each edge $vw$ of $T$ by the function $f_{wv}\from Q\to Q$ such that $f_{wv}(p)=q$ if $[w\mapsto p]\vdash [v\mapsto q]$. 
%
%Observe that if $w$ is any descendant of $v$ then $[w\mapsto p]\vdash [v\mapsto q]$  if and only if the composition of the functions labelling the edges along the path from $w$ to $v$ is a function $f$ such that $f(p)=q$. Hence, the data structure given by \cref{lem:reverse enumerate} gives the enumerators of the second type, as required in the statement. \sebi{need to ensure that $w\in X$}
\end{proof}





We now prove~\cref{lem:shape enumeration}.
\begin{proof}
    Fix a shape $\sigma$. The proof proceeds by induction on the size of the tree $S$ underlying $\sigma$.

    In the base case $|S|=1$ 
there may be at most one valuation $\tup a$ that matches $\sigma$ with a starting node~$v$, namely the valuation $\tup a\from\tup y\to V(T)$  that maps all the variables $\tup y$ of $\sigma$ to $v$. 
This valuation matches~$\sigma$ precisely whenever $\rho_v(v)=p$, where $\rho_v\from V(T)\to Q$ is the run of $\aut A$ on $T\otimes \tup a$
and $p=L(\ast)$. We use an automaton to label all vertices in a tree
that satisfy the desired conditions. 

\begin{claim}
  There is an automaton $\aut A'$ on augmented trees over the alphabet $A$ with states $Q_0\cup Q_1$ such that for any tree $T$,
  the run of $\aut A'$ on $T$
  labels a node $v$ of\, $T$ with a state in $Q_1$ if and only if $\rho_v(v)=p$.
\end{claim}
\begin{proof}
We use a similar construction as in \cref{lem:powerset construction}. 
For a tree~$T$ and $w\in V(T)$ let us write $T\otimes w$ to denote $T\otimes \tup a$, where $\tup a$ is the valuation mapping all variables of~$\bar y$ to $w$ (recall that in \cref{lem:powerset construction} we were
dealing with a single free variable only, however, the construction works
analogously if we map all variables to the same vertex). 
Again, for a tree $T$ and $w\in V(T)$ let $q(\aut A, T\otimes w)$ denote the state at the root of $T$ in the unique run of $\aut A$ 
on~$T\otimes v$. We construct the automaton $\aut A'$ as in 
\cref{lem:powerset construction} (but using the above definition of
$T\otimes w$), which uses the states $Q\times Q\times 2^Q\times 2^Q$
and every node $v\in V(T)$ gets labeled by the tuple
  $(q,q',N,R)$ with:
  \begin{align*}
    q&=q(\aut A,T_v\mathop{\otimes} \emptyset),&
                                                        q'&=q(\aut A, T_v \mathop{\otimes} v),\\
    N&=\setof{q(\aut A,T_v \mathop{\otimes} w)}{w\text{ is a child of $v$ in $T$}}&
                                                                                          R&=\setof{q(\aut A, T_v \mathop{\otimes} w)}{w\in V(T), v\prec w}.
  \end{align*}

By this construction, a node $v$ needs to be labeled by a state 
in $Q_1$ if and only if $q'=p$. We hence 
partition the state set into $Q_0$ and $Q_1$ by 
defining $Q_1$ as those tuples $(q,q',N,R)\in 
Q\times Q\times 2^Q\times 2^Q$ with $q'=p$. 
\end{proof}

We now output the following enumerators 
$(\mathcal E_v)_{v\in V(T)}$. For all $v\in Q_1$ we let
$\mathcal E_v$ be the enumerator that outputs the 
unique valuation mapping all variables in $\tup y$ to $v$, 
otherwise, $\mathcal E_v$ is the empty enumerator. 
This finishes the base case. 

\smallskip
Now assume $|S|>1$. Following the notation from
    above, we write $\ast$ for the root of $S$.
Let $W$ be the set of children of $\ast$ in~$S$.
%
% Fix a node $v\in V(T)$.
% Let $B_v$ be the set of all pairs $(G,H)$ where $G\from W\to \str A_v$ is an  injective mapping and $H\from W\to Q$,
% for which there is a function $F\from V(S)\to V(T)$
% satisfying conditions 1, 2, 4, 5 above,  with $F(w)\succeq G(w)$
% and $\rho(F(w))=G(w)$,
% for all $w\in W$
%
%
% \begin{claim}\label{claim:branching}
%     There is an algorithm that computes in time linear in $|T|$ for  each  $v\in V(T)$
%      an enumerator for $B_v$ with constant delay.
% \end{claim}
% \begin{proof}
    Fix  $w\in W$ %and $p\in Q$,
    and define a shape %$\sigma_w^p$
    $\sigma_w$ with the following components:
    \begin{itemize}
        \item the variables $\bar y_w:=\setof{y\in\tup y}{w\preceq \tup s(y)}$,
        \item the subtree $S_w$ of $S$
        rooted at $w$,
        \item the restriction $L_w$ of the labeling $L$ to $S_w$,
        \item the restriction $\tup s_w$ of the valuation $\tup s$ to $\tup y_w$.
    \end{itemize}


Note that $S_w$ has less nodes than $S$, so we can apply the inductive assumption to $\sigma_w$,
for each~$w\in W$.


Let $q$ be the label of the root in $S$ and let $\tup z\subset \tup y$ be the set of those variables $y\in \tup y$ such that $\tup s(y)$ is the root $\ast$ in $\sigma$.
Let $\rho_0$ be the run of $\aut A$ on $T\otimes \emptyset$.

%Fix functions $H,H'\from W\to Q$.
For a node $v\in V(T)$ with label $a$ and injective function $G\from W\to \str A_v$,
say that  $G$ is \emph{satisfiable} if there is a function $G'\from W\to\str A_v$ such that the  following conditions hold (recall that
$L$ also labels edges of $S$ and that $\ast w$ denotes the edge between the
root $\ast$ of $S$ and $w$):
\begin{itemize}
    \item
    $\delta_{q,(a,\tup z)}$ holds in $\str A_v$ labeled by $\rho_0$, except for the nodes $G(w)$ for $w\in W$ that are instead labeled by~$L(\ast w)$, 
    \item for each $w\in W$ we have
     $G'(w)\succeq G(w)$
    and $[G'(w) \mapsto L(w)]\vdash [G(w)\mapsto L(\ast w)]$, and
\item for each $w\in W$
 there is some valuation of $\bar y_w$ that matches $\sigma_w$ with
  starting node $G'(w)$.
\end{itemize}

\begin{claim}\label{claim:bijection}
    Valuations $\tup a$ that match $\sigma$ with starting node $v$
    are in bijective correspondence with tuples $(G,G',(\tup a_w)_{w\in W})$, such that $G,G'\from W\to \str A_v$ and:
    \begin{enumerate}
        \item $G$ is satisfiable,
        \item $G'(w)\succeq G(w)$ and $[G'(w)\mapsto L(w)]\vdash [G(w)\mapsto L(\ast w)]$ for all $w\in W$, and
        \item  $\tup a_w$ matches $\sigma_w$ with starting node $G'(w)$
        for all $w\in W$.
    \end{enumerate}
\end{claim}
\begin{proof}
    Fix a valuation $\tup a\from \tup x\to V(T)$ that matches $\sigma$ with starting node $v$ and let $\rho$ be the run of $\aut A$ on~$T\otimes \tup a$. As remarked above, the function $F\from V(S)\to V(T)$ witnessing that $\tup a$ matches
    $\sigma$ is unique.
    Define  $(G,G',(\tup a_w)_{w\in W}))$ as follows, by setting for $w\in W$:
    \begin{itemize}
        \item $G(w)$ is the $F(w)$-directed child of $F(\ast)$, % that is an ancestor of  $F(w)$,
        \item $G'(w)=F(w)$,
%        \item $H(w)=\rho(G(w))$,
%         \item $H'(w)=\rho(G'(w))$,
        \item $\tup a_w$ is the restriction of $\tup a$ to $\tup y_w\subset \tup y$.
    \end{itemize}

    As $\tup a$ matches $\sigma$ with starting node $v$, we have that
    $\rho(v)=q$ and
    the image of $\tup a$ is contained in the union of $\set v$ and the set of descendants of either of the nodes $G(w)$, for $w\in W$.
    Since the run $\rho$ is computed deterministically in a bottom-up fashion, it follows that the runs $\rho$ and  $\rho_0$ differ only on those vertices of $\str A_v$
    that are in the image of $G$.
Moreover, $\rho(G(w))=L(\ast w)$ by definition of $S$. As $\rho(v)=q$ it follows that the formula $\delta_{q,(a,\tup z)}$ holds in $\str A_v$ labeled by $\rho$.


Fix $w\in W$. We show that
  $\tup a_w$ matches $\sigma_w$ with starting node $G'(w)$.
To this end, it is enough to
%exhibit a function $F_w\from V(S_w)\to V(T)$ satisfying conditions 1-5 for the shape $\sigma^{H(w)}_w$. The
observe that the restriction $F_w$ of $F$ to $V(S_w)$ witnesses this.
%By construction, $F_w$ satisfies the required conditions, yielding the conclusion.
In particular, this
shows that  $G$ is satisfiable.

Vice versa, from a tuple $(G,G',(\tup a_w)_{w\in W})$ satisfying
the properties of the claim we uniquely obtain the valuation $\bar a$ 
matching $\sigma$ with starting node $v$: $\bar a=\bigcup_{w\in W}\tup a_w\cup \bar b$, where $\bar b$ is the valuation that maps~$\bar z$
(the set of variables $y\in \bar y$ such that $\bar s(y)=\ast$) to $v$. 

Hence, the assignment $\tup a\mapsto (G,G',(\tup a_w)_{w\in W})$ defined above yields the bijective correspondence as stated in the claim.
\end{proof}


The enumerator for the set of all valuations $\tup a$ that match $\sigma$ with starting node $v$
is obtained by enumerating all triples $(G,G',(\tup a_w)_{w\in W})$ that satisfy
the properties stated in the claim.
%All functions $H,H'\from W\to Q$ can be easily enumerated with constant delay.
%Fix such functions $H$ and $H'$.
We now argue that all components
can be enumerated with constant delay.

For $w\in W$,
let $X_w$ denote the set of nodes $u'$ such that there is a valuation that matches $\sigma_w$ with starting node $u'$. 
By inductive assumption, in particular we can compute $X_w$ in time linear in $|T|$.
Apply \cref{lem:state entailment} to
$T$ and $X_w$ and states $q_2=L(w)$ and $q_1=L(\ast w)$, to obtain, for each $v\in V(T)$, an enumerator for the set $C_w(v)$ of all children $u$ of $v$ such that there exists $u'\succeq u$ in $X_w$ satisfying \[[u'\mapsto L(w)]\vdash
[u\mapsto L(\ast w)].\]

For each child $u$ of $v$,
label $u$ by the set of all $w\in W$ such that $u\in C_w(v)$. This yields a labeling $\lambda_v$ of the whorl $\str A_v$.

Let $\tup w$ be the set $W$, where now each $w\in \tup w$ is treated as a variable.
Then there is a first-order formula~$\psi(\tup w)$ with free variables $\tup w$
that holds in $\str A_v$ with the  labeling $\lambda_v$ for a valuation $\tup b\from \tup w\to \str A_v$ if~$\tup b$
induces a function $G\from W\to \str A_v$ that is injective and satisfiable.
By assumption on the class~$\CC$,
we can compute an enumerator for the formula $\psi(\str A_v)$, for each $v\in V(T)$. % and each $H\from W\to Q$.
Each enumerator has delay bounded by some constant, and all those enumerators can be computed in time linear in $|T|$.
In particular, in this way we obtain for each $v\in V(T)$ an enumerator with constant delay that enumerates all satisfiable functions $G\from W\to\str A_v$.

Fix $v\in V(T)$ and a satisfiable function $G\from W\to \str A_v$. Our next task is to enumerate all functions $G'\from W\to\str A_v$ that certify satisfiability of $G$.
The key observation is that this can be done by enumerating, for each $w\in W$ independently, all nodes  $u'$ of $V(T)$ with $u'\succeq G(w)$ and \mbox{$[u'\mapsto L(w)]\vdash[G(w)\mapsto L(\ast w)]$},
and such that there is some valuation of $\tup y_w$ that matches $\sigma_w$ with starting node $u'$.
Note that this last condition is equivalent to $u'\in X_w$. Hence, for a fixed $w\in W$, it suffices to enumerate all descendants $u'\in X_w$
of $G(w)$ with  $[u'\mapsto L(w)]\vdash[G(w)\mapsto L(\ast w)]$.
This is done using the enumerator obtained from~\cref{lem:state entailment}.

More precisely,
for each $w\in W$, apply \cref{lem:state entailment} to
$T$ and $X_w\subset V(T)$ and states $q_2=L(w)$ and $q_1=L(\ast w)$, obtaining, for each $u\in V(T)$
an enumerator for the set $Y_w(u)$ all descendants  $u'\in X_w$ of $u$ that satisfy \[[u'\mapsto L(w)]\vdash
[u\mapsto L(\ast w)].\]

In particular, for $u=G(w)$ we obtain an enumerator for the set $Y_w(G(w))$ of all descendants~$u'$ of~$G(w)$ that belong to $X_w$ and satisfy the above. Now, functions $G'\from W\to V(T)$ that certify satisfiability of $G$ are exactly all functions $G'\from W\to V(T)$
such that $G'(w)\in Y_w(G(w))$, for all $w\in W$. Therefore, all such functions can be enumerated with constant delay, by taking the product of the enumerators of the sets $Y_w(G(w))$, for $w\in W$.


Hence, we may compute in time linear in $|T|$ a data structure that, given $v\in V(T)$, enumerates all pairs $(G,G')$ such that $G\from W\to \str A_v$ is satisfiable, and
$G'\from W \to V(T)$ certifies that.
Fix such a pair $(G,G')$.
It remains to construct a data structure that allows to enumerate all tuples $(\tup a_w)_{w\in W}$ such that $\tup a_w$ matches $\sigma_w$ with starting node $G'(w)$, for all $w\in W$. Again, this can be done by enumerating, independently for each $w\in W$, all valuations $\tup a_w$ that match $\sigma_w$ with starting node $G'(w)$.
Apply the inductive assumption to $\sigma_w$ for each $w\in W$,
yielding in time linear in $|T|$ for every node $u\in V(T)$
an enumerator with constant delay for the set $Z_w(u)$ of the set of all valuations $\tup a_w$ that match $\sigma_w$ with starting node $u$.
Then tuples $(\tup a_w)_{w\in W}$ as above are exactly the tuples in $\prod_{w\in W}Z_w(G'(w))$. Therefore, all such tuples may be enumerated with constant delay, by taking the product of the enumerators for the sets $Z_w(G'(w))$ for $w\in W$.

Reassuming, we may compute in time linear in $|T|$ a data structure that, given $v\in V(T)$, enumerates all triples $(G,G',(\tup a_w)_{w\in W})$ that satisfy the condition of~\cref{claim:bijection}. Those correspond precisely to tuples~$\tup a$ that match $\sigma$ with starting node $v$,
as described in the claim. This yields the conclusion of the inductive step, and finishes the proof of~\cref{lem:shape enumeration}.
\end{proof}

% \begin{proof}
%     Let $\phi(\tup x)$ be a first-order formula.
%     We describe an efficient enumeration algorithm
%     for $\phi$.
% We proceed by induction on $|\tup x|$.
% The base case, when $\tup x$ is empty, is handled by~\cref{thm:formula evaluation}.

% Consider the inductive step, and fix any variable $x\in\tup x$.
% By inductive assumption, we can efficiently enumerate all valuations $\tup a$ satisfying the formula $\exists x.\phi(\tup x)$.
% Fix any such valuation $\tup a$. The goal now is to enumerate efficiently all vertices $v$ such that
% the valuation $\tup av$ satisfies $\phi(\tup x)$.
% Consider $\tup a$ as constants, by considering the tree $T\otimes \tup a$. We therefore need to enumerate all nodes $v\in V(T)$  that satisfy the formula $\phi(x)$
% in $T\otimes \tup a$,
% where the symbols in $\tup x$ are now treated as constants.
% To simplify notation, we assume henceforth that $\tup x$ is empty.\sz{The whole proof below needs to be fixed}

% Let $\aut A$ be the automaton obtained from $\phi$ as described in~\cref{thm:formulas to automata}, so that the following conditions are equivalent, for any node $w$ of $T$:
% \begin{itemize}
%     \item $\phi(w)$ holds in $T$,
%     \item $\aut A$ accepts $T\otimes w$.
% \end{itemize}





% Let $\rho$ be the run of $\aut A$ on $T\otimes \emptyset$. For
% a vertex $w$ and state $q\in Q$,
% define the labelling $\rho[w\mapsto q]$
% of the vertices in $V(T)$ which are not descendants of $w$,
% such that $\rho[w\mapsto q](v)$ is equal to $\rho(v)$ if $v\neq w$ and is equal to $q$ if $v=w$. Say that $\rho[w\mapsto q]$ is \emph{accepting} if it labels the root node with an accepting state, and for every node $v$ with letter $a$ and such that $w\not\preceq v$, the state $q=\rho(v)$ is such that $\delta_{q,a}$ holds in the $Q$-labelled whorl at $v$, with labelling $\rho[w\mapsto q]$.



% Consider now the  automaton $\aut A'$ from~\cref{lem:powerset construction}, and let $\rho'$ be the run of $\aut A'$ on $T$. This run can be computed in time linear in $|T|$, by~\cref{lem:automata evaluation}.
% Let $\rho$ be the run of $\aut A$ over $T\otimes \emptyset$.
% \begin{claim}For every node $v$ of $V(T)$,
%     $\aut A$ accepts $T\otimes w$
%     for some child $w$ of $v$
%     if and only if
%     $\rho[v\mapsto q]$ is accepting for
%     some $q\in \rho'_3(v)$, where $\rho'_3(v)$ is the third component of $\rho'(v)$.
% \end{claim}
% \begin{proof}
%     For right-to-left implication,
%     suppose $\rho[v\mapsto q]$ is accepting
%     for some $q\in\rho'_3(v)$.
%     By definition of $\rho'_3(v)$, there is a child $w$ of $v$ such that $\aut A( T_v \otimes w)=q$.
%     We construct a run of $\aut A$ on $T\otimes w$.
%     This run labels every node $u$ other than $w$ with $\rho(u)$, and labels $w$ with
%     $\aut A(\subtree T w\otimes w)$.
%     This is an accepting run of $\aut A$ on $T\otimes w$, proving one implication.
%     The other implication is similar.
% \end{proof}


% Let $\pi\from V(T)\to 2^Q$
% be such that  every node $v\in V(T)$
% is labelled by the  set $\pi(v)$ of all states $q\in \rho'_3(v)$ such that
%     $\rho[v\mapsto q]$ is accepting.


% \begin{claim}
%     There is an automaton $\aut B$ on augmented trees with states $\wh Q$ and a function
%     $f\from \wh Q\to 2^Q$ such
%     that for every augmented tree $T$ and run $\gamma$ of $\aut B$ on $T$,
%     $f\circ \gamma$ is the labelling $\pi$ described above.
% \end{claim}
% \begin{proof}
%     \sz{prove, using product construction}
% \end{proof}



% Let $X$ be the set of all nodes $v\in V(T)$ such that $\pi(v)$ is nonempty.
% We can enumerate all nodes $v\in X$ with constant delay.
% \sz{Need: enumeration algorithm for an \MSO formula $\phi(\tup y,x)$ which performs linear-time preprocessing and given a tuple $\tup y$ enumerates all $x$'s satisfying $\phi$ with constant delay.}

%  It remains to enumerate all children $w$ of any given $v\in X$ such that $\aut A$ accepts $T\otimes w$.
% \begin{claim}Fix $v\in X$ and a child $w$ of $v$. Then
%     $\aut A$ accepts $T\otimes w$ if and only if there is some $q\in\pi(v)$ such that
%     $\phi_{q,\emptyset}$ holds in the whorl at $v$ labelled by $\rho$, except for $w$ which is labelled by $\aut A(\subtree T w\otimes w)$.
% \end{claim}


% For $v\in X$ and $q\in \pi(v)$, let
% $X_{v,q}$ be the set of
% all children $w$ of $v$ such that
%     $\phi_{q,\emptyset}$ holds in the whorl at $v$ labelled by $\rho$, except for $w$ which is labelled by $\aut A(\subtree T w\otimes w)$.

% \begin{claim}
%     The set $X_{v,q}$ can be efficiently enumerated.
% \end{claim}

% Our final enumeration algorithm works as follows.
% \begin{enumerate}
%     \item Enumerate all $v\in X$.
%     \item For each $v\in X$ and each $q\in \pi(v)$, enumerate the set $X_{v,q}$, and output each $w$ in this set.
% \end{enumerate}

% \end{proof}


==> mc-unbreakable.tex <==
\section{Model-checking on unbreakable classes}

\textcolor{red}{We think that the proof goes slightly differently. It is not sufficient to 
statically evaluate $\conn(u,v,s_1,\ldots, s_k)$ using the oracle. Instead
it should go like this. }

Prove the more general version of \cref{thm:formula enumeration}. 

\begin{theorem}\label{thm:conn formula enumeration}
    Suppose enumeration of \FOsep-queries is efficient on $\CC$. 
    Then enumeration of \FOsep-queries is efficient on $\CC$-augmented trees.
\end{theorem}

Now prove that we can efficiently evaluate $\FOsep$-queries on 
$H$-topological-minor free unbreakable graphs and conclude. 

\begin{lemma}
Let $\phi$ be an $\FOsep$ formula and let $k$ be the maximum arity
of a separator atom in $\phi$. Let $\Dd$ be a class such that 
$\FO$ model-checking is fpt linear on $\Dd$. Let $\Cc$ be the
$(q(k),k)$ unbreakable fragment of $\Dd$. Then $\phi$ can be 
evaluated in linear time on $\Cc$. 
\end{lemma}
\begin{proof}
We show that $\phi$ is equivalent on $\Cc$ to an FO formula and 
use the model-checking algorithm for FO on $\Dd$. 

As $G\in \Cc$ is $(q(k),k)$ unbreakable for every set $S$ of size at
most $k$ that is deleted from $G$ only one connected component
has more than $q(k)$ vertices. Hence, vertices $u$ and $v$ are connected 
in $G-S$ if and only if they are connected by a path of length at most 
$q(k)$ or both $u$ and $v$ are in a (the unique) component of size
greater than $q(k)$ (unless all components are small, then we are in the
first case). Both properties are easily expressible in FO using 
$q(k)$ quantifiers. 
\end{proof}

\begin{remark}
$\FOsep$ queries on unbreakable classes of bounded expansion are hence 
checkable in linear time. This seems like a contradiction to the hardness
on some classes of bounded expansion. The reason is that we 
crucially use that we can contract the components of the children of a 
bag and preserve the property that the resulting bag graph excludes a 
topological minor. This is not the case in classes of bounded expansion. 
\textcolor{red}{How does the decomposition of the $n$-subdivison of
an $n$-clique look like?}
\end{remark}
